Dynamics-Guided Diffusion Model for Sensor-less Robot Manipulator Design

We present Dynamics-Guided Diffusion Model (DGDM), a data-driven framework for generating task-specific manipulator designs without task-specific training. Given object shapes and task specifications, DGDM generates sensor-less manipulator designs that can blindly manipulate objects towards desired motions and poses using an open-loop parallel motion. This framework 1) flexibly represents manipulation tasks as interaction profiles, 2) represents the design space using a geometric diffusion model, and 3) efficiently searches this design space using the gradients provided by a dynamics network trained without any task information. We evaluate DGDM on various manipulation tasks ranging from shifting/rotating objects to converging objects to a specific pose. Our generated designs outperform optimization-based and unguided diffusion baselines relatively by 31.5% and 45.3% on average success rate. With the ability to generate a new design within 0.8s, DGDM facilitates rapid design iteration and enhances the adoption of data-driven approaches for robot mechanism design. Qualitative results are best viewed on our project website https://dgdm-robot.github.io/.

==> text/approach_rebuttal.tex <==
\section{Approach}


% \begin{figure*}
%     \centering
%     % \includegraphics[width=\textwidth]{imgs/approach.png}
%     % \caption{We employ a dynamics network that predicts interaction dynamics, from which objective gradients can be constructed based on user task specifications. Then the gradients are used to guide the denoising process of a diffusion model to generate the desired end-effector shapes.}
%     \includegraphics[width=\textwidth]{figures/method_v2.jpg}
%     \vspace{-0.3cm}
%     \caption{
%         \textbf{DP$^2$} consists of a diffusion model over Bezier control points for the finger mesh (a), and a dynamics models which predicts the delta-translation and rotation conditioned on the object point cloud, initial object poses, and the finger control points (b).
%         Finally, by defining task-specific manipulation objectives over the predicted delta-dynamics (c), gradients from these objectives can flow back through the task-agnostic delta-dynamics model to update the finger control points.
%         \todo{``(c) manipulation objectives'' looks quite empty. Not sure how to fill up space. Legend looks too big. Object point cloud not very clear. Does object mesh need to be there?}
%     }
%     \vspace{-0.5cm}
%     \label{fig:method}
% \end{figure*}



\input{text/task_specification_v1}

\subsection{Dynamics Network}
\label{sec:dynamics}
% We propose to model interaction dynamics between the manipulator and object with a dynamics network to efficiently and flexibly provide gradients to guide designs. 
% We propose to predict interaction profiles with a dynamics network to efficiently and flexibly provide gradients to guide designs.
The dynamics network $\mathcal{D} : (o,m,p) \mapsto \Delta p$ aims to learn a general model of how a random distribution of fingers interacts with a distribution of objects.
Importantly, it provides gradients of the design objective with respect to the finger representation \textcolor{red}{(Fig.~\ref{fig:method})}.
The following paragraphs describe the details of the dynamics network's training procedure.

\textbf{Shape Representation.}
We choose cubic Bézier curves and surfaces as the shape representation \textcolor{red}{of} the manipulator for their flexibility and ubiquity in parameterizing shapes~\cite{fitter2014review}. 
Control points are grid sampled along the length (and height in 3D) of the finger while the remaining y-coordinate of the control points determines its protrusion outwards/inwards. \textcolor{red}{The y-coordinates of the control points are used as $m$ (the geometry parameter of manipulator).}
We represent object shape $o$ as a point cloud by surface sampling the object mesh.
For 2D objects, we sample 100 2D points from their contour surfaces.
For 3D objects, we sample 512 3D points from all surfaces.


\textbf{Motion Representation.}
We represent object motion under interaction as a three-dimensional vector consisting of delta rotation along the z-axis, delta translation along the x-axis, and delta translation along the y-axis, denoted as $\Delta p=(\Delta\theta,\Delta x,\Delta y)$. 
% The dynamics network is denoted as $\mathcal{D}: (o, m, p)\mapsto\Delta p$, where $o$ is the object shape, $m$ is the manipulator shape vector, and $p=(\theta, x, y)$ denotes the initial object configuration in $\mathbf{SE}2$ space.

\textbf{Network Architecture.}
In the 2D manipulation case, we use an MLP as the network architecture.
First, we transform sampled object initial poses $p$ with a high-frequency positional encoding - a trick typically used to combat over smoothing of neural networks~\cite{mildenhall2021nerf}.
Then, $o$ and $m$ are passed through separate 2-layer multi-layer perceptrons (MLPs) with 256 hidden dimensions, before being concatenated together with the high-frequency pose embedding.
Finally, the resulting embedding is passed through an 8-layer MLP with 256 hidden dimensions to get the predicted object motion $\Delta p$.
In 3D, we use a PointNet++~\cite{qi2017pointnet++} encoder to encode object geometry, whereas all other parts of the architecture are shared between 2D and 3D tasks. 


\textbf{Training Data Generation.}
% \huy{Most important thing to emphasize is that this happens \emph{once for all tasks}}
Since our dynamics network training only requires task-agnostic data, its data generation happens once for all tasks.
We sample random object and manipulator pairs, load them into MuJoCo~\cite{todorov2012mujoco} simulation environment, and measure $\Delta p$ after a single parallel jaw closing interaction.
% The network is trained with simulation data generated in MuJoCo~\cite{todorov2012mujoco} environment.
For the 2D case, we generate 321 planar object shapes by first extracting contours of 2D icon images from the Icons-50 dataset~\cite{hendrycks2018robustness}, and then extruding it to a planar shape.
In the 3D setting, we select 164 objects from Google's Scanned Objects Dataset~\cite{downs2022scannedobjects, zakka2022scannedobjectsmujoco}, filtering out objects whose scales are out of bound or tilt over during interaction.
We randomly sample 1024 manipulator geometry parameters $m$ from a uniform distribution.
For each object-fingers pair, we grid sample 360 initial orientations and 5$\times$5 initial positions, then run forward simulations to get delta object poses after a single gripper close.
In total, we use 321$\times$1024$\times$360$\times$25 data points for training the 2D dynamics network and 164$\times$1024$\times$360$\times$25 data points for training the 3D dynamics network.

\textbf{Design Objective Gradient Evaluation.}
To design manipulators that are generalizable to more initial poses $p$ and objects $o$, the design objective $F$~\eqref{eq:shift_up_aggregate} can be evaluated for a wider range of poses and objects.
Concretely, we can grid-sample $p$'s and a set of $o$'s and evaluate each motion objective $f$ in parallel along the batch dimension.
The design objective gradient $\nabla_m F$ is attained by aggregating the gradients along the pose/object batch dimension.
For each new design, evaluating $\nabla_m F$ takes 0.16 seconds on average, which makes it efficient to run in the inner loop of iterative design procedures.
In this project, we grid-sample 360 orientations and 5$\times$5 positions, getting a 360$\times$5$\times$5 dimensional motion profile.

\textbf{Modelling Interactions instead of Modelling Contacts.}
Differentiable simulators~\cite{xu2021end, li2023learning, wang2024diffusebot, spielberg2019learning, hu2019chainqueen} are another popular choice for providing $\nabla_m F$, but suffer from two major limitations.
First, soft contact models, such as penalty-based methods used by \citeauthor{xu2021end}, are known to yield biased and high-variance gradients~\cite{suh2022pathologies, li2023learning}.
Further, such gradients need to be computed for each simulation timestep, which is computationally expensive for long-horizon interactions.
Instead of modeling individual contacts as in differentiable simulators, our dynamics network learns to capture the temporally extended finger-object interaction.
This data-driven approach can be trained on physically accurate simulated data, avoiding the limitations associated with soft contacts.
Moreover, our dynamics network exhibits flexibility by seamlessly generalizing to novel objects and tasks at test time, allowing for the construction of objectives without extra data generation/training.


\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/method_rasterize_1-a.pdf}
    \caption{
        \textbf{\fullname.}
        % make sure notation in the figure is consistent with the final version in the paper
        Our approach generates finger shapes given a target object and task, specified as a target interaction profile (\S~\ref{sec:task}) describing how the object should move under different initial configurations.
        This target can be compared with the dynamics network's prediction of the current interaction profile, which is used to construct a differentiable objective (\S~\ref{sec:dynamics}).
        Gradients of the objective are then used to iteratively guide the reverse denoising process of a manipulator shape diffusion model (\S~\ref{sec:diffusion}).
        By averaging gradients across more sampled poses and target objects, our framework can generate fingers that are robust to a wider range of initial poses and tailored to more objects.
    }
    \label{fig:method}
\end{figure}


\subsection{Dynamics-Guided Diffusion Model}
% \todo{in this entire section, maybe use k instead of t for diffusion timestep, so it matches figure}
\label{sec:diffusion}
Given design objective gradients from $\mathcal{D}$ (\S~\ref{sec:dynamics}), the obvious approach is to perform gradient descent on the finger geometry~\cite{xu2021end,ha2021fit2form,taylor2019optimal,kodnongbua2022computational,li2023learning}.
However, the distribution of good designs are often multi-modal, which means gradient descent approaches quickly get stuck in local minima.
Instead, to efficiently navigate through the large and multi-modal design space, we extend classifier guidance~\cite{dhariwal2021diffusion}, an iterative diffusion model sampling approach that enables a balance between multi-modal diversity and task-specific guidance \textcolor{red}{(Fig.~\ref{fig:method})}.

% The diffusion model is trained on an unconditional shape parameter distribution, and guided with the task-specific objective gradients towards desired designs.

\textbf{Diffusion Model.}
Diffusion models~\cite{sohl2015deep, ho2020denoising} are a class of probabilistic generative models that generate samples from an underlying distribution through iterative denosing. A diffusion model $\epsilon_\theta(m_k)$ predicts the noise added to a sample~\cite{ho2020denoising}, which is trained by first adding noise $\epsilon$ to $m_0$ to produce noised sample $m_k$, and then apply a mean-squared error loss between the ground truth noise and predicted noise $||\epsilon_\theta(m_k)-\epsilon||^2$. To generate samples from a diffusion model, we start with a Gaussian noise $m_K$ and gradually predict less-noisy samples $m_{K-1}, m_{K-2}, ...,$ until final sample $m_0$. The process involves repeatedly predicting $m_{k-1}$ from $m_{k}$, which is the reverse noising process of modeling the distribution $p_\theta(m_{k-1}|m_{k})$.
Specifically, we employ Denoising Diffusion Implicit Models (DDIMs)~\cite{song2020denoising} as the sampling method.

We sample \textcolor{red}{geometry parameters of manipulator} $m$ from a uniform distribution and train a diffusion model on this distribution. The diffusion model $\epsilon_\theta(m_k)$ with 1D UNet architecture~\cite{ronneberger2015u} predicts noise added to a sample $m_k$. We use DDIM for diffusion sampling process $p_\theta(m_{k-1}|m_{k})$ with 15 training denoising iterations and 5 inference iterations, and the Square Cosine noise scheduler~\cite{nichol2021improved}.


\textbf{Background on Classifier Guidance.}
Many techniques are developed to condition diffusion model on certain inputs or guide the reverse diffusion process with priors, such as concatenation, cross-attention~\cite{rombach2022high}, classifier-free guidance~\cite{ho2021classifier}, \etc. Among these approaches, classifier guidance~\cite{dhariwal2021diffusion} can guide the reverse noising process towards desired samples with an unconditional diffusion model.
It requires a classifier $p_\phi(l|m_k)$, where $m_k$ is the sample, $l$ is the class label, and $\phi$ is the classification network. To condition the sampling process on label $l$, each reverse noising transition is:
\begin{equation}
    p_{\theta, \phi}(m_k|m_{k+1},l) = Zp_\theta(m_k|m_{k+1})p_\phi(l|m_k)
\end{equation}
where $Z$ is a normalizing constant.
Classifier guidance can be applied to DDIM sampling method. Leveraging the connection between diffusion models and score matching proposed by~\cite{song2020improved, song2020score}, a score function for $p(m_k)$ can be derived from the diffusion model:
\begin{equation}
    \nabla_{m_k}\log p_\theta(m_k)=-\frac{1}{\sqrt{1-\bar{\alpha_k}}}\epsilon_\theta(m_k)
\end{equation}

where $\alpha_k\coloneqq1-\beta_k, \beta_k$ is the variance of Gaussian noise added to samples at denoising step $k$, and $\bar{\alpha_k}\coloneqq\prod_{s=1}^k\alpha_s$.
The score function for $p_\theta(m_k)p_\phi(l|m_k)$ is:
\begin{equation}
    \begin{split}
        \nabla_{m_k}\log(p_\theta(m_k)p_\phi(l|m_k)) = \nabla_{m_k}\log p_\theta(m_k) + \nabla_{m_k}\log p_\phi(l|m_k)\\
        = -\frac{1}{\sqrt{1-\bar{\alpha_k}}}\epsilon_\theta(m_k) + \nabla_{m_k}\log p_\phi(l|m_k)
    \end{split}
\end{equation}

A new noise prediction can be defined as:
\begin{equation}
    \hat{\epsilon}(m_k)\coloneqq\epsilon_\theta(m_k)-\sqrt{1-\bar{\alpha_k}}\nabla_{m_k}\log p_\phi(l|m_k)
\end{equation}
Then DDIM can be performed with the modified noise prediction for conditioned sampling.

\textbf{Dynamics Guidance \& the Effects of Guidance Scaling.}
To guide the design generation towards manipulation design objectives, we extend classifier guidance to use interaction profiles instead, which we term dynamics guidance.
% In doing so, dynamics guidance relaxes diffusion model training requirements to make use of 
Concretely, we replace classifier gradients with $\nabla_{m_k} F(m_k)$ to guide the DDIM sampling process (Algo.~\ref{dynamicsguide}).
% We further condition the dynamics network on diffusion sampling timestep and train with corresponding noisy samples: $\mathcal{D}: (o, m_k, p, k)\mapsto\Delta p$.  shows our dynamics guidance procedure.
% \huy{this following sentence just repeats information from the previous paragraph}
% By tuning the hyperparameter $s$, the scale of gradients, we can trade-off between diversity and fidelity~\cite{dhariwal2021diffusion}. With a larger gradient scale, the generated distribution becomes sharper, producing samples with higher fidelity but less diversity. 
% \todo{justify it's a re-normalized distribution or change the notation to probability?}
% Tab.~\ref{tab:objectives} shows how the classifier gradients for primitive and complex objectives are constructed. Note that $\nabla\log p(\cdot)$ abbreviates for $\nabla_{x_t}\log p(\cdot|x_t)$, $i$ denotes different initial poses. \todo{regression model formulation}
By extending classifier guidance, we not only enable guiding unconditional diffusion models with task-specific gradients, but also inherit an elegant way to trade off diversity and performance.
% The classifier gradients can be scaled to tune the sharpness of sample distribution~\cite{dhariwal2021diffusion}. 
Since $s\nabla_{m}\log p(l|m)=\nabla_{m}\log \frac{1}{Z}p(l|m)^s$, where $s$ is the gradient scale and $Z$ is an constant, increasing $s$ has the effect of sharpening the sampling distribution towards $p(l|m)^s$.
\citet{dhariwal2021diffusion} showed that when $s$ is larger the distribution becomes sharper and generated samples have higher fidelity, while smaller scale leads to more diverse samples.
We observe the similar effect of different gradient scales~\cite{dhariwal2021diffusion} from our generated results, as shown in Fig.~\ref{fig:diffusion}.


\begin{algorithm}[t]
    \caption{Dynamics guided DDIM sampling, given a diffusion model $\epsilon_\theta(m_k)$, design objective $F(m_k)$ constructed from dynamics network, and gradient scale $s$.}
    \begin{algorithmic}
        \State Input: design objective $F(\cdot)$, gradient scale $s$
        \State $m_K \gets \text{sample from~} \mathcal{N}(0, \mathbf{I})$
        \ForAll{$k$ from $K$ to $1$}
        \State $\hat{\epsilon} \gets \epsilon_\theta(m_k) - s\sqrt{1 - \bar{\alpha}_k} \nabla F(m_k)$
        \State $m_{k-1} \gets \sqrt{\bar{\alpha}_{k-1}} \left(\frac{m_k - \sqrt{1-\bar{\alpha}_k}\hat{\epsilon}}{\sqrt{\bar{\alpha_k}}} \right) + \sqrt{1 - \bar{\alpha}_{k-1}}\hat{\epsilon}$
        \EndFor\\
        \Return $m_0$
    \end{algorithmic}
    \label{dynamicsguide}
\end{algorithm}



==> text/eval_rebuttal.tex <==

\section{Evaluation}

We design\textcolor{red}{ed} experiments and a suite of manipulation tasks, aimed at answering the following questions:
\begin{enumerate}
    \item Does our approach design effective manipulators customized for a range of unseen tasks and 2D/3D objects?
    \item Does dynamics-guided diffusion generation provide better performance than gradient descent optimization? What are the design strategies the algorithm learns? 
    \item How does different conditioning (\eg, multiple objects) impact the final design?  
    \item How do designs from our approach transfer to real hardware?
\end{enumerate}

\textbf{Manipulation Tasks \& Metrics.}
\textcolor{red}{We evaluated each approach on held-out objects (8 in 2D, 6 in 3D) and manipulation tasks.
Each pair of fingers is mounted to a WSG50 gripper performing a fixed open-close action.}
We categorize our suite into two difficulty levels.
\begin{enumerate}
    \item \textbf{Primitive objectives} involve single-axis object movements or rotations in $SE2$ space, \textcolor{red}{including shifting up, shifting down, shifting left, shifting right, rotating clockwise, and rotating counterclockwise. For each object-manipulator pair, we grid-sampled 360 planar initial object orientations and performed fixed open-close actions with the manipulator. The task is considered as successful if the movement of the object along the axis of focus is larger than a predefined threshold. For example, a manipulator designed for the rotating counterclockwise objective succeeds if it can rotate the object a degree larger than a threshold after the first open-close action. Then, we report the average success rate over all sampled initial object orientations.}
    \item \textbf{Complex objectives} combine multiple primitive objectives to parameterize a broad range of manipulation tasks.
          \textcolor{red}{T}he convergence objective includes rotation objectives with target directions and magnitudes based on initial object orientation. \textcolor{red}{W}e report the \textcolor{red}{maximum convergence range} in degrees, indicating the broadest range of initial \textcolor{red}{object} orientations \textcolor{red}{that can be driven towards a consistent final orientation within a small tolerance (5 degrees) \textcolor{red}{by the manipulator}. \textcolor{red}{Observing continued object movement, we report convergence metrics after the 40th open-close manipulator action.}
          Additionally, we explore\textcolor{red}{d rotate clockwise and shift up, rotate clockwise and shift left, and rotate either way} objectives to showcase our approach's flexibility in composing orthogonal or conflicting objectives.
          \textcolor{red}{These} tasks \textcolor{red}{were} evaluated on \textcolor{red}{average} success rates.
\end{enumerate}


\textbf{Ablations.}
First, removing our task-specific guidance from our dynamics model yields the \textbf{Unguided} baseline, which generates task-agnostic manipulators using our geometry diffusion model.
Second, removing our diffusion model yields the \textbf{Opt.} baseline, which optimizes the manipulator control points using gradients of the task objective through our dynamics network, common for many prior works~\cite{ha2021fit2form,xu2021end, li2023learning, kodnongbua2022computational}.
To mitigate performance variance due to initialization, we \textcolor{red}{ran} each approach 16 times per object-task pair and select\textcolor{red}{ed} the best performance, then average\textcolor{red}{d} among objects. \textcolor{red}{Results are reported in Tab.~\ref{tab:single_result}, Tab.~\ref{tab:multi_result} and Fig.~\ref{fig:results_prim}.}

\input{tables/table_singleobj.tex}
\input{tables/table_multiobj.tex}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/results_prim_rasterize-a.pdf}
    \caption{\textbf{Results on Primitive Objectives.}
        We generate manipulators for primitive objectives that involve motion along one dimension in $SE2$ space. Red and green object masks denote object configurations before and after interaction respectively, overlaid with the image after closing in the manipulator. Compared with baseline methods, finger shapes produced by our method achieve the task much more effectively.
    }
    \label{fig:results_prim}
    \vspace{-5mm}
\end{figure*}


\subsection{Experiment Results}
\subsubsection{\textbf{Task-specific manipulators}}
\label{sec:eval:task_specific}
Despite having no task-specific training, our dynamics and diffusion model can generate tailored fingers for a wide variety of scenarios, surpassing the unguided baseline (\ie, uniform control points) \textcolor{red}{across all primitive and complex tasks}.
The advantages of generating custom fingers over random counterparts become more pronounced as the design requirements escalate.
For instance, our approach exhibit\textcolor{red}{ed} a $+16.6\%$ improvement over the unguided baseline in 2D primitive objectives, a figure that expand\textcolor{red}{ed} to $20.0\%$ in 2D complex objectives (see Tab.~\ref{tab:single_result}).
A similar trend \textcolor{red}{was} observed when transitioning from 2D to 3D objects ($+18.0\%$ over Unguided in 2D, $+23.4\%$ over Unguided in 3D, Tab.~\ref{tab:single_result}) and from single-object to multi-object designs ($+18.0\%$ over Unguided in single-obj 2D, $+18.6\%$ over Unguided in multi-obj 2D, Tab.~\ref{tab:multi_result}).

In each of these scenarios, where task complexity, design space, and the target object set grow, a human expert designer would face significantly increased time and effort.
However, our approach, leveraging the gradient aggregation from individual motion objectives (per initial configuration, task, and object), offers a simple yet effective solution to handle progressively complex design requirements.
As long as users can articulate how \emph{each} object should move from \emph{each} initial pose, this specification can be seamlessly incorporated into the diffusion denoising process.


\begin{figure}[h]
    \centering
    \includegraphics[width=0.49\textwidth]{figures/diffusion_rasterize-a.pdf}
    \vspace{-0.4cm}
    \caption{
        \textbf{Effect of Scaled Guidance.}
        % We model the task- and object-agnostic design space with a diffusion process on the manipulator bezier control points (a). 
        From left to right we increase scaled guidance in the diffusion process. The increased scale will enforce more task guidance and achieve higher task performance (shifting down), however, reduce the diversity of generated designs. By tuning this parameter, the user could trade-off between diversity and task guidance of the candidate designs at test time.
    } \vspace{-3mm}
    \label{fig:diffusion}
\end{figure}
\subsubsection{\textbf{Robustness \& efficient search with guided diffusion}}
\label{sec:eval:diffusion_diversity}
The Opt. baseline and \ours share the same task objective gradients from our learned dynamics network, differing only in how this gradient information is incorporated.
The baseline uses gradient descent, a method that requires upwards of 18 and 24 minutes to converge in 2D and 3D (for 16 samples), respectively, and is prone to local minima.
In contrast, our approach utilizes classifier-guidance with a diffusion denoising process, which strikes a balance between exploring different modes (by introducing Gaussian noise) and exploiting the current mode (using the gradient of design objective) through a guidance scaling factor (Fig.~\ref{fig:diffusion}).
This results in $+12.8\%$ and $+10.4\%$ higher success rates than the baseline in 2D and 3D primitive objectives, respectively.
Additionally, our diffusion models prove stable even with diffusion processes as short as 5 timesteps, translating to an average design time of 13 and 54 seconds in 2D and 3D (for 16 samples), respectively.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/results_convergence_rasterize-a.pdf}
    \caption{
        \textbf{Convergence Results.}
        For each pair of finger designs, we show the range of initial orientations (``cvrg. range'') which converges to the same convergence mode (``cvrg. target'').
        In the generated designs (under ``ours''), we observe two emergent design patterns: a bulge on one finger pushes the object into the other finger with a hollow cavity (a,b,d-f,h), and two parallel surfaces on either finger ``catch'' and align objects with symmetric flat edges (c,g). In both strategies, the pair of fingers must simultaneously exploit object \textbf{geometry} and \textbf{physics} (sliding) and coordinate their own geometry to achieve the most effective convergence.
        %This emergent coordination between the pair of finger designs all emerged from the dynamics guidance and is not common in the baseline.
        % \huy{cvrg. range and cvrg. target or "init" and "final"? I prefer latter}
    }
    \label{fig:results_convergence}
\end{figure*}

\subsubsection{\textbf{Emergent design for convergence}}
\label{sec:eval:convergence_strategies}
What strategies do our designs employ to consistently achieve convergence from a broader range of initial orientations compared to the unguided baseline ($+21.3^\circ$ in 2D, $+8.9^\circ$ in 3D, Tab.~\ref{tab:single_result})?
From Fig.~\ref{fig:convergence}, we identify two emergent design patterns not commonly observed in the baseline algorithm:
\begin{enumerate}
    \item \textbf{Push-and-Catch}: In the majority of our convergence designs, one finger features a bulge that pushes the object into the hollow cavity of the other finger (Fig.~\ref{fig:results_convergence} a,b,d-f,h).
          Interestingly, this cavity should \textcolor{red}{roughly} complement the object's size and shape at the convergence point, but not precisely.
          We hypothesize that this extra wiggle room (most prominent in Fig.~\ref{fig:results_convergence} e,f) supports a broader range of initial orientations by allowing extreme orientations to ``slide'' into the optimal orientation, caught by the cavity.
    \item \textbf{Parallel-Align}:
          When objects exhibit symmetric flat edges, our designs utilize two parallel surfaces on each finger to align these edges (Fig.~\ref{fig:results_convergence} c,g).
          Here, the parallel surfaces not only align with the object's flat edges but also with each other, reinforcing the object from both sides towards the target convergence orientation.
\end{enumerate}
In both of these strategies, the pair of fingers must simultaneously exploit object \textcolor{red}{geometry} (\ie, size, shape, symmetry) and \textcolor{red}{physics} (sliding), coordinating their geometry to achieve the most effective convergence.
This emergent coordination between the pair of finger designs arise\textcolor{red}{d} from our dynamics guidance and is not commonly observed in the baseline.
%\todo{symmetry and multiple convergence mode?}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/result_multiobject_rasterize-a.pdf}
    \caption{
        \textbf{Specialized or Generalized Design in Multi-object Scenarios.}
        Our approach can be flexibly conditioned on individual objects and generate a specialized design for each object [Top] or simultaneously conditioned on multiple objects at once and generate one design for all objects [Bottom]. 
        This flexibility allows the user to trade-off between performance (single-object) and generality (multi-object) based on the task and system requirements. 
    }
    \vspace{-3mm}
    \label{fig:results_multi}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/result_real_rasterize-1-a.pdf}
    \caption{
        \textbf{Real-world Results.} We manufacture manipulators generated by \ours and execute the open-loop parallel closing motion. Behaviors in simulation successfully transfer to the real world. 
        Red and green masks denote object configurations before and after interaction respectively.
        % Red and green object masks denote object configurations before and after interaction respectively, overlaid with the image after closing in the manipulator.
    }
    \label{fig:results_real}
\end{figure*}

\subsubsection{\textbf{Specialized or generalized designs for multi-object scenarios}}
\label{sec:eval:multiobj_strategies}
It is commonplace for automation pipelines to handle various object types with differing geometries.
In such cases, opting for a more generic design that performs well across all objects may be advantageous, as opposed to fabricating one optimal design for each object.
However, customizing manipulators for multiple objects quickly becomes unwieldy, as a gripper designed to achieve the task with one object might cause undesirable effects on another object.
For example, a manipulator pair designed to rotate a T-shape clockwise could inadvertently move a house- and car-shaped object up without rotation (Fig.~\ref{fig:results_multi}, top row, `rotate clockwise').

Approaching this challenge from a compositional perspective intuitively appears promising, requiring two key skills.
First, the designer must enumerate a \textcolor{red}{diverse set of design candidates} that achieve the task for each object, including designs that may not be optimal.
Second, the designer must sift through these candidates to prioritize common design patterns effective across all objects.
Ultimately, these common elements can be composed into a unified design suitable for all considered objects.
In other words, design approaches unable to navigate a large, multi-modal design space or filter through a vast set of design candidates may struggle to achieve this multi-object design scenario.

Our algorithm demonstrates the ability to discover this compositional design intuition by effectively balancing diversity (\S~\ref{sec:eval:diffusion_diversity}) with object- and task-specific performance guidance (\S~\ref{sec:eval:task_specific}).
From Fig~\ref{fig:results_multi}, we observe that the multi-object fingers for ``shift down'' (first column) combine the left finger from one design and the right finger from another design.
Meanwhile, the left multi-object finger for ``rotate clockwise'' is derived from the left single-object finger for the house.
In contrast, the unguided baseline lacks task-specific guidance, hindering its ability to guide its diverse generations toward a common design effective for all objects.
On the other extreme, the Opt. baseline often gets stuck in a local minimum, unable to effectively explore a multi-modal design space.
These limitations are reflected in Tab.~\ref{tab:multi_result}, with our approach achieving $+18.6\%$ and $+23.4\%$ higher success rates than the unguided baseline in 2D and 3D, respectively, and $+14.7\%$ and $+17.6\%$ higher success rates than the Opt. baseline in 2D and 3D, respectively.

Naturally, we acknowledge that multi-object finger designs must sacrifice some performance compared to the single-object scenario ($-1.5\%$ in 2D, $-5.2\%$ in 3D) to achieve more object-level generality.
This balance between generality and task-specific performance is a fundamental trade-off in mechanism design in automation, with the optimal compromise dependent on the specific application.
These results illustrate that designs from our approach can vary along this spectrum without additional training, providing a valuable tool for designers to explore the trade-off in their design space.




% Thanks to our bezier curve parameterization, our generated fingers are directly 3D printable.
% These printed fingers are mounted on a real world WSG50 gripper (Fig.~\ref{fig:results_real}).
% low cost, rapid iteration cycle,
% Results are best demonstrated in video, in the supplementary material.
% dynamics guidance: gradient scale, number of initial pose samples, number of finger shape initialization samples, optimizing control points or all up-sampled points
\subsubsection{\textbf{Real-world evaluation with Sim2Real transfer}}
We show real-world results of all tasks for both 2D and 3D cases by mounting the 3D printed designs on a WSG50 \textcolor{red}{gripper produced by WEISS ROBOTICS} (Fig.~\ref{fig:results_real}). \textcolor{red}{The 3D printer we use is Creality Ender-3 S1 and its molding solution is FDM. The material we use for 3D printing objects and fingers is PLA.}
\textcolor{red}{In Tab.~\ref{tab:real} we report quantitative metrics for target objects and grippers shown in Fig.~\ref{fig:results_real} compared with results in simulation. For the shifting down, shifting right, and rotating counterclockwise tasks, we sample 10 different initial poses of the object in real (360 different initial poses in simulation) and report the average success rate ($\%$). For the convergence task, the maximum range of initial orientations ($\degree$) that can be driven to the target convergence pose is reported.}
Surprisingly, our Sim2Real transfer was significantly simplified due to our sensor-less formulation - with no perception and closed-loop control, only geometry and physics impacted the transferability.
Overall, our real-world results highlight the robustness of our designs to unmodeled plastic deformations in simulation and manufacturing imperfections.
For instance, our convergence fingers typically achieve convergence much faster in the real world because the lower friction coefficient of 3D printing PLA material allows the object to slide into the cavity more easily (\S~\ref{sec:eval:convergence_strategies}).
These results are best viewed in the video attached in the supplementary material.

\begin{table}
    \centering
    \caption{
        \textcolor{red}{\textbf{Real-world Quantitative Results.} We report quantitative results for 3D printed manipulators and compare with corresponding simulation results on various tasks.}
    }
    \footnotesize
    \setlength\tabcolsep{2.5pt}
    {\color{red}\begin{tabular}{cc|cc|cc|cc|cc}

        \toprule
        \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{Shift Down} & \multicolumn{2}{c|}{Shift Right} & \multicolumn{2}{c|}{Rotate Counter} & \multicolumn{2}{c}{Convergence}\\
        \multicolumn{2}{c|}{} & sim & real & sim & real & sim & real & sim & real\\
        \midrule

        \multirow{3}{*}{2D}
                              & T                                  & 93.1                                   & 90                 & 100                  & 100                  & 75.3                    & 70                   & 111$\degree$                    & 124$\degree$\\
                              & Heart                                      & 78.3                                   & 80                 & 99.2                  & 100                  & 66.1                    & 70                   & 117$\degree$                    & 119$\degree$\\
        \midrule

        \multirow{3}{*}{3D}
                              & Chair                                  & 91.4                                   & 100                 & 100                  & 100                  & 68.6                    & 70                   & 93$\degree$                    & 86$\degree$\\
                              & Basket                                      & 96.9                                   & 100                 & 100                  & 100                  & 65.3                    & 70                   & 82$\degree$                    & 88$\degree$\\
        \bottomrule
    \end{tabular}}
    \label{tab:real}
\end{table}


\section{Conclusion and future directions} 
We present \fullname, a versatile framework for the rapid generation of diverse and tailored manipulator geometry designs for unseen tasks.
This task-agnostic framework lays the groundwork to enable more rapid experimentation and future research.
To expand the scope of our work beyond geometry design, investigating co-optimizing articulation structure, materials, and policy would unlock broader applications.
To support a better interface for users, it is an interesting future direction to automatically detect when different objectives conflict with each other (\eg, in multi-object scenarios) using their gradients, and informing the user on the feasibility of the design requirements.

\textcolor{red}{
\ours can be applied to many useful applications. The manipulator designed for convergence can be used as a part feeder for part assembly. By combining a series of shifting/rotating operations with manipulators generated by our framework, we can apply precise motion to the object. The framework can be further applied to design problems beyond 2D manipulation. For example, it may be applied to articulated robots and soft robots design, morphing structure design, etc.}
We hope that our framework contributes to the wider adoption of data-driven approaches in the domain of robotic mechanism design.

==> text/huy_notes.tex <==
# Alternate motivation for our modules

1) How to flexibly support specification of objectives/parameterize task space?
When thinking about learned components which can be reusable in all/many/most tasks, we must decide what the shared "API"/structure between them are.
Ideally, this shared structure should be minimal - such that it's easy to use.
However, this minimalism should also provide sufficient flexibility to parameterize the task space we care about.
This allows the user to specify the objective.

2) How to enable efficient and robust search?
The second is how to enable efficient yet robust search within that objective.
Grid/Uniform-random search's robustness to non-convex design landscapes comes at the cost of brute-force simulation.
Meanwhile, gradient-based optimization could require many regularization terms to ensure a well-behaved optimization procedure but still often gets stuck in local-minima.

So, within the space of manipulation tasks, what is the shared structure, and how
In other words, how can we "prompt" generative models to design task-specific grippers?

Our framework, Neural Morphological Design, answers these two questions with two respective modules: ...

# related works reading

Optimization for robot hardware design.
When have a model and have a good initialization, gradient-based optimization could be the most efficient way.
However, when lots of complex contact modes are involved, gradient-based optimization can be tricky.

\subsection{Robot End-effector design}

\subsection{Geometry optimization for robot hardware design}
First-order gradient optimization of morphology only~\cite{wolniakowski2015task} or both morphology and control~\cite{taylor2019optimal}, but requires careful initialization and suffers from local minima.
Zeroth-order optimization using graph heuristic tree search, or model predictive path integral (MPPI) evolutionary algorithms have been explored for co-optimization of morphology and control~\cite{zhao2020robogrammar}, but requires careful design of the search space (via recursive graph grammar~\cite{zhao2020robogrammar}) to remain tractable.
All optimization approaches typically include many regularization terms or hand crafting of the design space to ensure well-behaved optimization dynamics and tractability respectively, which are all task-specific and difficult to adapt to new tasks.

~\cite{kodnongbua2023computational} for special cases where only concerned with material properties, compliance, and weight, then can use topology optimization, but not generally applicable.

~\cite{xu2021end} actually does fully end-to-end gradient-based optimization of morphology and control.
However, enabling contact-rich manipulation using differentiable simulators is tricky - differentiable penalty-based approaches are known to yield bad gradients in contact-rich manipulation cases where it's close to discontinuous~\cite{suh2022pathologies}.
(used 4 tasks, finger reach, flip box, rotate rubik's cube, and assemble), separate optimization for each task.
Each task itself requires a costly optimization procedure.
However, with every new task, the user must design new objectives and regularizations, start optimization from scratch, without leveraging any of the previous optimization experience.


To automate the process, previous works have explored leveraging optimization algorithms for robot hardware design.
\cite{wolniakowski2015task} optimizes gripper geometries parameterized by cuboids using various quality metrics.
\cite{taylor2019optimal} co-optimizes the curvature of end-effector shape and motion trajectory to improve the throwing distance.
RoboGrammar~\cite{zhao2020robogrammar,xu2021multi, hu2023glso, hu2022modular} co-optimize robot topology and control parameters of arthropod robots to cross terrains with graph heuristic search over robot designs generated by a recursive graph grammar.
To automatically design passive grippers that can grasp objects without additional actuation, \cite{kodnongbua2023computational} co-optimizes passive gripper geometry represented with skeleton and inserting trajectory.
DiffHand~\cite{xu2021end} and \cite{li2023learning} optimize geometries of robots or tools for robots by deforming an initial shape using cage-based deformation with gradients from a differentiable simulator. However, differentiable simulators yield bad gradients in contact-rich manipulation cases where it's close to discontinuous~\cite{suh2022pathologies, li2023learning}.

% single-task optimization, heavily engineered objective functions
% require shape initialization, high-dimensional design parameter, local minima, struggle with large-multimodal design space, cannot efficiently explore full design space
These works deal with single-task optimization and require heavily engineered objective functions that cannot be reused for new tasks. They also struggle with efficiently navigating through the design space, especially when good initializations are not available and the design space is high-dimensional and multi-modal.

\subsection{Data-driven robot hardware design} % task-specific data

Fundamentally, data-driven approaches enables sharing of experiences in one scenario to another, thus inference time/optimization costs.
One popular data-driven approach is to distill the evaluation process into a value network, which takes as input the embodiment parameterization and outputs the task-specific performance of the design.
This strategy has been applied to guide graph search in designing locomotion robots~\cite{zhao2020robogrammar,xu2021multi} and grippers~\cite{ha2021fit2form}.
When co-optimizing morphology and control, \cite{wang2019neural} uses each evaluation trial to train an embodiment-conditioned controllers, such that the performance of each morphology design can be more quickly and accurately evaluated.

\cite{zhao2020robogrammar,xu2021multi} learns embodiment/multi-objective weight value networks to guide graph search (since their design space is a combinatorial design topology space).
In contrast, we focus on the task of optimizing parameterized geometry, and thus, we can leveraged gradients from learned modules to guide the generation process.
Taking this further, \cite{wang2019neural} uses each evaluation trial to train an embodiment-conditioned controllers, such that the performance of each morphology design can be more quickly and accurately evaluated.
However, the data collection process is often expensive, and the data is often task-specific.


For instance, within gripper design~\cite{ha2021fit2form} and locomotion~\cite{hu2023glso}, a large complex design space is compressed into a small, continuous latent space using Variational Auto-encoders, then gradient descent is performed in the latent space to optimize the design.
In both these cases, the design space encoder is trained with task-agnostic design candidates, but the value network used to guide this design optimization is trained with task-specific data.
However, this approach requires a large amount of \emph{existing} task-specific data to train the VAE, and the latent space is not guaranteed to be smooth and continuous, which can lead to poor optimization performance.

It is also typical to cycle between data collection and learning, similar to an actor-critic setup in reinforcement learning.
% in {xu2021multi}, it is separated into 3 phases on repeat: design phase, evaluation phase, and learning phase.
Both \citeauthor{ha2021fit2form} and \citeauthor{xu2021multi} use this approach, where they collect data with a current policy, then train a new policy with the collected data.

Exploring multi-modal design spaces is a challenging yet important problem.
For instance, within modular robotics design optimization~\cite{hu2022modular}, where the morphological combination is combinatorial, learning one-to-many mappings is ideal.
They used GANs~\cite{goodfellow2014generative}, which are notoriously difficult to train stably.

Prior works have shown that morphology and control be co-optimized.
In locomotion over rough terrain, and in passive grasping.
Why don't we do it?

# method pass
NMD - chinese swear word, also doesn't add much, vague

words use sparingly but not explained:
 - global/local objectives

notation: object V to O?

one more figure to show how to compose/decompose objectives? visual => math

\mathcal{D} is defined twice with two conflicting definitions (with/without t). I think this should be fine?

do differentiable simulators actually require analytical gradients each time?

==> text/intro.tex <==
\begin{abstract}
    abstract goes here
\end{abstract}

\twocolumn[{%
            \renewcommand\twocolumn[1][]{#1}%
            \maketitle
            \vspace{-5mm}
            \begin{center}
                % \includegraphics[width=\textwidth]{figures/Design_Teaser.pdf}
                % \captionof{figure}{\textbf{Neural Mechanical Design.} our xxx algorithm learns to generate different end-effector geometry to achieve different manipulation goals with a fixed end-effector motion (i.e., closing in parallel).  For example, achieving specified object movement (e.g., move up) for one or multiple objects or achieving object pose converging after a sequence of interactions.  Note: The link to the figure draft is in the link below (comment), feel free to edit or update directly}
                %https://docs.google.com/drawings/d/1wUrv389b8zm7cN-PHxjADk5-uZXNQlELRV_mm9lLO0Y/edit?usp=sharing
                \includegraphics[width=\textwidth]{figures/teaser_v5.jpg}
                \captionof{figure}{\textbf{Neural Morphological Manipulator Design.}
                    Given input objects (a), our algorithm learns to generate manipulators that achieves the desired objectives (b-d) with a fixed open-loop gripper motion (i.e., closing in parallel).
                    From simple objectives (b-c) to complex ones (d), and single objects (top two rows) to the multi-object scenario (bottom row), our framework can be output diverse design candidates without further training or simulation, enabling fast design iteration cycles.
                }
                % https://www.figma.com/file/FZwZHVBhacPcyHzSiLr2bY/Scaling-Up-Distilling-Down?type=design&node-id=798%3A943&mode=design&t=79h9q1k9i2pTh8Nf-1
                % TODO looks too empty, waste of space
            \end{center}
        }]


\section{Introduction}
\label{sec:intro}
% What's Mechanical intelligence, and why it is important 
Mechanical intelligence~\cite{} refers to the use of morphological design, material systems, and physical phenomena to solve tasks and adapt to new situations and tasks.
Much evidence in both natural~\cite{beal2006passive} and artificial systems~\cite{mcgeer1990passive} have demonstrated that a well-customized embodiment to a particular environment or task could greatly simplify an agent's learning, control, and decision-making process, improving its overall performance and robustness~\cite{pfeifer2009morphological}.

Despite its benefits, mechanical intelligence in robotics has recently been overshadowed by the rapid development of its counterpart, ``action intelligence'', where agents with a fixed embodiment are endowed with complex control schemes.
Recent advancements in data-driven approaches such as reinforcement learning~\cite{levine2016end,schulman2017proximal} and behavior cloning~\cite{chi2023diffusionpolicy,zhao2023learning} have demonstrated policies that generalize to novel tasks, environments, and even new embodiments~\cite{huang20d,feng23a}.
% At the same time, there has been a lot of recent progress in applying diffusion models in text-conditioned image generation~\cite{ho2020denoising}, greatly outperforming generative adversarial networks~\cite{goodfellow2014generative} and variational auto-encoders~\cite{}, in terms of generation diversity, scalability to high resolution images, and training stability.
% Here, despite sparse data distributions over test-time text labels, diffusion-based approaches exhibit a remarkable ability to generalize from diverse training data.

What has prevented morphological design from enjoying similar benefits of machine learning?
We identify two key challenges:
\begin{itemize}
    \item \textbf{Task-specific data is sparse:}
          Tailoring a morphological design for its exact use case (specific objects and objectives) is the key to achieving better performance and robustness.
          However, the data for a specific task is often sparse, and recollecting training data for every application scenario is too expensive to be practical.
          As a result, most of the prior work focuses on single task optimization~\cite{ha2021fit2form} or relies on heavily engineered objective functions that could not be reused for new tasks~\cite{xu2021end, li2023learning, schaff2019jointly, hu2022modular, luck2020data, chen2020hardware}.
    \item \textbf{Large, Multi-modal Design Spaces:}
          To sidestep the problem of navigating large design spaces, most prior works assume good initializations for optimization~\cite{ha2021fit2form,xu2021end, li2023learning, kodnongbua2023computational}, which are non-trivial to obtain and limits the possible design output candidates.
          Further, as the design space grows, the landscape of ones that perform well in a particular task typically becomes more multi-modal.
          % explain how returning diverse candidates can help allow the designer to try the next most promising design when the top candidates fail due to domain gap
          Exploration of the most promising modes and the ability to return diverse sets of near optimal candidates are crucial.\todo{huy: still have to argue for domain gap, explore design problem, and why diverse candidates are important}
\end{itemize}


In this paper, we study data-driven morphological design in the context of manipulation.
We introduce \textbf{Dynamics-Guided Diffusion-based Generation} (DG$^2$), a framework that learns to generate diverse end-effector geometry designs for a parallel jaw gripper to achieve different manipulation tasks with novel objects.
Its design output can be conditioned on varying numbers of objects and ranges of initial configuration without further retraining, providing a user-controllable knob to trade-off generality and performance.

% \todo{add the key insight of the paper here}
Our key insight is that a differentiable objective over learned dynamics
when using dynamics as the shared structure between tasks, we could use powerful generative architectures to explore the large multi-modal design space.
From this insight, our key contribution is an extension of classifier-guided diffusion-based generation~\cite{dhariwal2021diffusion}, which enables the usage of a task-agnostic dynamics model to guide the diffusion process.
This formulation inherits the benefits of diffusion models, including the ability to generate diverse, multimodal outputs and training stability, while enabling the generation of task-specific manipulators without the need for task-specific training/data (e.g., task-success classifiers).
To support our key contribution, our framework consists of two components:
\begin{itemize}
    \item \textbf{Dynamics Network}:
          % In contrast to differentiable simulators, whose gradients suffer from bias from soft contact formulations~\cite{suh2022pathologies} in contact-rich scenarios, our learned dynamics model can be trained over any complex physical scenarios.
          %   By modelling the object interaction dynamics in a differentiable manner, we can use the dynamics model's output to define differentiable manipulation objectives.
          % for modeling general interaction dynamics ...
          % + Models object interaction dynamics in a differential manner
          % + General dynamics can be combined and used to model complex object
          %   for modeling general interaction dynamics between the manipulator and object. 
          The delta-dynamics network takes object shape and manipulator shape as input and predicts the design ``profile" -- delta poses of the object under all possible initial configurations. Different task objectives can be constructed by combining the general dynamics for different initial poses, different moving directions, and across multiple objects. This dynamics network is fully differentiable, and thus gradients of the objective with respect to the manipulator shape can be calculated, indicating the directions of desired designs in the design space.

    \item \textbf{Geometry Diffusion Model}:
          % for modeling the design space with ..
          for modeling the design space of manipulator shapes. It is trained on the general manipulator shape distribution without any task conditions. During test time, we use the objective gradients provided by the dynamics network to guide the diffusion model's denoising process, enabling the generation of desired designs for novel objects and flexible objectives.

\end{itemize}

% We implement this algorithm with ... [more details about the algorithm...]

In the end, with an extremely simple control scheme -- closing the two end-effectors in parallel, the same model generates manipulator designs that achieve drastically different manipulation goals, including specified object motion objectives under different initial poses, as well as complex objectives that require reasoning about sequential interactions such as convergence~\ref{fig:finger}.
% Thanks to its flexible design, the same model could be employed for 
%Learning to generate task-specific design without task-specific training 


% \todo{Maybe it's better to motivate from diffusion models in image generation and ask why its not obvious to apply classifier guidance for task-specific design.}
We demonstrate results on both 2D and 3D objects with generated 2D and 3D manipulators. We test on primitive, complex, single-object and multi-object manipulation objectives under a sensorless setting, where the initial pose of the object is arbitrary and unknown. Results in simulation and the real world demonstrate that designs generated by DG$^2$ achieve high task performance, with a $-\%$ average improvement compared to unguided diffusion generation results.


==> text/intro_rebuttal.tex <==

% \twocolumn[{%
%             \renewcommand\twocolumn[1][]{#1}%
%             \maketitle
%             \vspace{-5mm}
%             \begin{center}
%                 % \includegraphics[width=\textwidth]{figures/Design_Teaser.pdf}
%                 % \captionof{figure}{\textbf{Neural Mechanical Design.} our xxx algorithm learns to generate different end-effector geometry to achieve different manipulation goals with a fixed end-effector motion (i.e., closing in parallel).  For example, achieving specified object movement (e.g., move up) for one or multiple objects or achieving object pose converging after a sequence of interactions.  Note: The link to the figure draft is in the link below (comment), feel free to edit or update directly}
%                 %https://docs.google.com/drawings/d/1wUrv389b8zm7cN-PHxjADk5-uZXNQlELRV_mm9lLO0Y/edit?usp=sharing
%                 \includegraphics[width=\textwidth]{figures/teaser_rasterize_1-a.pdf}
%                 \captionof{figure}{\textbf{
%                         % \ours for Robot Manipulator Design.
%                         Task-specific Designs without Task-specific Training.
%                     }
%                     Given input objects (a), our algorithm learns to generate diverse manipulator geometries tailored to unseen manipulation tasks (b), which can be deployed with an open-loop motion (c) (\ie, closing in parallel).
%                     Our framework generates designs for new tasks and objects in seconds, unlocking rapid design iteration cycles. % <= this sentence feels unfinished. it's missing a part here that goes something like ".. unlocking rapid design iteration cycles for data-driven mechanical design"
%                     % Without the need for task-specific training or data generation, our framework generates designs within seconds, enabling fast design iteration cycles.
%                 }
%                 \label{fig:teaser}
%             \end{center}

%         }]
\vspace{-5mm}
\begin{center}
    % \includegraphics[width=\textwidth]{figures/Design_Teaser.pdf}
    % \captionof{figure}{\textbf{Neural Mechanical Design.} our xxx algorithm learns to generate different end-effector geometry to achieve different manipulation goals with a fixed end-effector motion (i.e., closing in parallel).  For example, achieving specified object movement (e.g., move up) for one or multiple objects or achieving object pose converging after a sequence of interactions.  Note: The link to the figure draft is in the link below (comment), feel free to edit or update directly}
    %https://docs.google.com/drawings/d/1wUrv389b8zm7cN-PHxjADk5-uZXNQlELRV_mm9lLO0Y/edit?usp=sharing
    \includegraphics[width=\textwidth]{figures/teaser_rasterize_1-a.pdf}
    \captionof{figure}{\textbf{
            % \ours for Robot Manipulator Design.
            Task-specific Designs without Task-specific Training.
        }
        Given input objects (a), our algorithm learns to generate diverse manipulator geometries tailored to unseen manipulation tasks (b), which can be deployed with an open-loop motion (c) (\ie, closing in parallel).
        Our framework generates designs for new tasks and objects in seconds, unlocking rapid design iteration cycles. % <= this sentence feels unfinished. it's missing a part here that goes something like ".. unlocking rapid design iteration cycles for data-driven mechanical design"
        % Without the need for task-specific training or data generation, our framework generates designs within seconds, enabling fast design iteration cycles.
    }
    \label{fig:teaser}
\end{center}


% todo: try giving a different term to the dynamics model. we can predict the complete interaction profile between finger and object for all initial poses. this makes repeated use of a dynamics model. 
% in order to reuse the same learned modules, we have to ask the following key question: (if repeated dynamics network is one answer, and diffusion geometric prior is the other, then what are the questions?)
% predicts the complete design profile.
% learning-based approaches must first acknowledge the intricacies of human-designed mechanisms and the wide range of manipulation tasks which smart mechanical design aims to solve
% this means to ensure the learned component can be reused, we must find a common structure between tasks as different as pose convergence and sorting.

    %This involves learning it once and then adapting it at test time to new tasks and objects simply by specifying the desired interaction targets (\ie, how the manipulator should move each object from each initial pose).
    %To enable interaction targets to guide geometry designs, we propose Dynamics Guidance - an extension of classifier-guidance~\cite{dhariwal2021diffusion} designed to support gradients from manipulation objectives.
\begin{abstract}
    We present \fullname (\ours), a data-driven framework for generating manipulator geometry designs for a given manipulation task. Instead of training different design models for each task, our approach employs a learned dynamics network shared across tasks. For a new manipulation task, we first decompose it into a collection of individual motion targets which we call target interaction profile, where each individual motion can be modeled by the shared dynamics network. The design objective constructed from the target and predicted interaction profiles provides a gradient to guide the refinement of finger geometry for the task. This refinement process is executed as a classifier-guided diffusion process, where the design objective acts as the classifier guidance. We evaluate our framework on various manipulation tasks, under the sensor-less setting using only an open-loop parallel jaw motion. Our generated designs outperform optimization-based and unguided diffusion baselines relatively by $31.5\%$ and $45.3\%$ on average manipulation success rate. With the ability to generate a design within 0.8 seconds, our framework could facilitate rapid design iteration and enhance the adoption of data-driven approaches for robotic mechanism design.
\end{abstract}

\section{Introduction}\label{sec:intro}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/teaser_cvgr_rasterize_1-a.pdf} \captionof{figure}{
        \label{fig:convergence}
        \textbf{The Convergence Task.}
        Throughout this paper, we use convergence as an illustrative example.
        The goal of convergence is to design fingers that always reorient a target object to a specified orientation $\theta_{\textrm{target}}$ when closing the gripper in parallel.
        In industrial settings, this task is useful because it funnels the objects from arbitrary poses to a small set of $\theta_{\textrm{target}}$, thereby simplifying downstream perception/planning.
        Despite its utility, designing for convergence can be highly counter-intuitive.
        An experienced engineer may take many design cycles to develop a reasonable design for just one object and must repeat this process for each new object.
        In contrast, our framework generates a functional design for a novel object within seconds, all without any prior training specific to this task.
    } \vspace{-4mm}
\end{figure*}
% \huy{
%     % Change task-specific to specialized (or some other word that doesn't have a negative connotation)
% }

% What's Mechanical intelligence, and why it is important 
Mechanical intelligence refers to the utilization of mechanical design to solve tasks and adapt to new challenges~\cite{lu2021mechanical}.
A substantial body of evidence in both natural~\cite{beal2006passive} and artificial systems~\cite{mcgeer1990passive} has demonstrated that well-customized embodiments can significantly simplify an agent's perception and control, thereby enhancing overall robustness~\cite{pfeifer2009morphological}.

Despite its advantages, mechanical intelligence in robotics has recently been overshadowed by the rapid development of its counterpart, ``action intelligence'', where the agent focuses on inferring different actions for different tasks, assuming a fixed mechanical embodiment design.
Namely, recent advancements in data-driven approaches~\cite{chi2023diffusionpolicy} have demonstrated action intelligence that can be directly applied to novel tasks and environments.

In contrast, learning for mechanical design has largely focused on single task optimization~\cite{ha2021fit2form, wang2024diffusebot} or heavily engineered objective functions that could not be reused for new design task~\cite{xu2021end, li2023learning, schaff2019jointly, hu2022modular, luck2020data, chen2021hardware}.
In practice, this means automating task-specific design typically involves recollecting training data for every scenario, which is too expensive to be practical. Therefore, we investigate the following question:
\begin{center}
    \textcolor{red}{Can we automate task-specific mechanical design \\without task-specific training?}
\end{center}

% what it can do
We introduce \textbf{\fullname}, a framework that generates manipulator geometry designs in seconds, with no task-specific training and no perception - only a parallel jaw closing motion.
From tasks as simple as object translation to complex tasks requiring sequential interactions such as pose convergence (Fig.~\ref{fig:convergence}), our framework's designs achieve drastically different manipulation goals with geometry changes that are highly adapted to the task and object.
% segway into some details
To enable task-agnostic pretraining for task-specific designs, our framework consists of two key technical contributions, each answering a key research question:
\begin{itemize}
    \item \textbf{How to represent the task space?}
          The task representation has to be expressive enough to capture the wide range of manipulation tasks while being compact enough to be readily learned from data.
          Our key insight is that many manipulation tasks can be \textcolor{red}{decomposed} into a collection of individual motion targets that specify how \textcolor{red}{each} object should move under \textcolor{red}{each} initial pose. We call the collection of individual motions \textcolor{red}{interaction profile}. While the final composed objective is specific to the task, each of the individual motions can be modeled by a generic dynamics model that is reusable across tasks. %In this work, we model these individual dynamics using a neural network. 
    \item \textbf{How to facilitate efficient and robust search?}
          As the design space grows, the distribution of good designs often becomes multi-modal \textcolor{red}{(\ie, there are often multiple good design solutions to achieve a task)}, and the task of generating promising yet diverse design candidates becomes challenging.
          To address this issue, we propose a \textcolor{red}{dynamics-guided diffusion model}.
          % To efficiently search the design space and generate diverse solutions, 
          First, with the dynamics network, we can infer the {current} interaction profile for an object and the {current} fingers.
          The design objective constructed by comparing the current with the target (\ie, task-specific) interaction profiles gives us a gradient on how to update the finger.
          This guidance is incorporated into diffusion denoising steps similarly to classifier guidance~\cite{dhariwal2021diffusion}.
          Tuning the guidance scale allows users to trade off the exploration of diverse candidates and the exploitation of the most promising modes.
\end{itemize}

We demonstrate results on both 2D and 3D objects with a variety of manipulation objectives ranging from primitive to complex and single- to multi-object objectives, all under a sensor-less setting, where the initial pose of the object is unknown.
Experiments in simulation and the real world demonstrate that designs generated by our approach achieve high task performance, with $31.5\%$ and $45.3\%$ relative success rate improvements compared to optimization and unguided diffusion generation results.

% Different task objectives can be constructed by combining the general dynamics for different initial poses, different moving directions, and across multiple objects.
% This dynamics network is fully differentiable, and thus gradients of the objective with respect to the manipulator shape can be calculated, indicating the directions of desired designs in the design space.

==> text/related_rebuttal.tex <==
\section{Related work}


\subsection{Manual End-effector Design}
Domain-specific end-effector designs have a long history in robotics, which expands the system's capabilities while simplifying perception and control.
% \textcolor{red}{Manipulator designs can be categorized into serial/parallel based on the disposition of the degrees of freedom, and dexterous/underactuated based on the degrees of actuation.}
\textcolor{red}{The diverse array of manipulator designs we see today, including serial versus parallel, from dexterous to underactuated,} typically start as the result of many trail-and-error iterations by expert engineers.
\textcolor{red}{Heavy manual efforts are needed} to discover optimal and occasionally counter-intuitive designs in practice, which significantly hinders the development of designs for new applications.
For instance, for complex manipulation tasks such as convergence (Fig.~\ref{fig:convergence}), previous works only deal with 2D planar polygons, utilizing manual or analytical designs of grasping policy~\cite{goldberg1993orienting, aceituno2023certified} or gripper geometry~\cite{zhang2002gripper}.

\subsection{Analytical Optimization for Automatic End-effector Design}
To alleviate the manual efforts, previous works have explored optimization approaches to manipulator design.
Though non-linear optimization is possible~\cite{taylor2019optimal}, this approach typically requires careful task-specific formulation of objectives and constraints.
Therefore, first-order optimization of morphology only~\cite{wolniakowski2015task} or both morphology and control~\cite{taylor2019optimal,xu2021end,kodnongbua2022computational} is more common, but requires careful initialization (task-specific parameterization~\cite{wolniakowski2015task}, cage-based deformation~\cite{xu2021end,li2023learning}, or heuristics~\cite{kodnongbua2022computational}).
% Since gradient-based optimization is prone to local minima, careful design and initialization of the optimization variables  is required to ensure a well-behaved optimization procedure.
Further, tasks involving complex contact modes, such as the ones we consider, are known to yield biased and high variance gradients in differentiable simulators~\cite{suh2022pathologies, li2023learning}.
Importantly, all manual efforts involved in setting up an optimization problem are typically not transferrable to new tasks or objects, and thus require a significant amount of manual labor for each new task.


\subsection{Data-driven Robot Hardware Design}
Fundamentally, data-driven approaches offer an improvement over optimization-based approaches by facilitating the transfer of knowledge from one scenario to another, thus reducing costs at inference and optimization stages.
A common approach to leveraging data is to distill the evaluation process into a value network, which takes the embodiment parameterization as input and outputs the design's task-specific performance.
This value network can then be used to guide a search/optimization procedure, which is often more efficient than evaluating the design in simulation.
This direction has been explored in the realm of gripper design~\cite{ha2021fit2form} and locomotion~\cite{zhao2020robogrammar,xu2021multi}, to guide optimization~\cite{ha2021fit2form,hu2023glso,wang2024diffusebot} or graph search~\cite{zhao2020robogrammar,xu2021multi, hu2022modular,whitman2020modular}.
Another common approach is to learn a generative model of the design space, which effectively compresses the design space into a low-dimensional continuous latent space.
This makes offline optimization via gradient-descent~\cite{ha2021fit2form,hu2023glso} or online optimization via trial-and-error rollouts of random latent-space samples~\cite{ha2021fit2form,hu2022modular,wang2024diffusebot} significantly more efficient.
Finally, when co-optimizing morphology and control, leverage control experience from prior embodiment evaluations can significantly improve the efficiency and accuracy of new embodiment evaluations~\cite{schaff2019jointly,chen2021hardware}.

All these data-driven approaches require task-specific data, yet only work well when provided with enough data for robust generalization.
We posit that this requirement on a large amount of task-specific data has hindered the mass adoption of data-driven approaches to robot hardware design.
In this work, we aim at eliminating the requirement on task-specific data when designing manipulators for a new task, by leveraging dynamics as the shared structure between manipulation tasks.



